Measurement of K0S, Lambda, Antilambda production at HERA

The production of the neutral strange hadrons $K^{0}_{S}$, $\Lambda$ and $\bar{\Lambda}$ has been measured in $ep$ collisions at HERA using the ZEUS detector. Cross sections, baryon-to-meson ratios, relative yields of strange and charged light hadrons, $\Lambda$ ($\bar{\Lambda}$) asymmetry and polarization have been measured in three kinematic regions: $Q^2 > 25 \gev^2$; $5 < Q^2 < 25 \gev^2$; and in photoproduction ($Q^2 \simeq 0$). In photoproduction the presence of two hadronic jets, each with at least $5 \gev$ transverse energy, was required. The measurements agree in general with Monte Carlo models and are consistent with measurements made at $e^+ e^-$ colliders, except for an enhancement of baryon relative to meson production in photoproduction.

==> DESY-06-226-ref.tex <==
{
\def\bibname{\Large\bf References}
\def\refname{\Large\bf References}
\pagestyle{plain}
\ifzeusbst
  \bibliographystyle{./BiBTeX/bst/l4z_default}
\fi
\ifzdrftbst
  \bibliographystyle{./BiBTeX/bst/l4z_draft}
\fi
\ifzbstepj
  \bibliographystyle{./BiBTeX/bst/l4z_epj}
\fi
\ifzbstnp
  \bibliographystyle{./BiBTeX/bst/l4z_np}
\fi
\ifzbstpl
  \bibliographystyle{./BiBTeX/bst/l4z_pl}
\fi
{\raggedright
\bibliography{./BiBTeX/user/syn.bib,%
              ./BiBTeX/bib/l4z_articles.bib,%
              ./BiBTeX/bib/l4z_books.bib,%
              ./BiBTeX/bib/l4z_conferences.bib,%
              ./BiBTeX/bib/l4z_h1.bib,%
              ./BiBTeX/bib/l4z_misc.bib,%
              ./BiBTeX/bib/l4z_old.bib,%
              ./BiBTeX/bib/l4z_preprints.bib,%
              ./BiBTeX/bib/l4z_replaced.bib,%
              ./BiBTeX/bib/l4z_temporary.bib,%
              ./BiBTeX/bib/l4z_zeus.bib}}
}
\vfill\eject


==> DESY-06-226-tab.tex <==
%-------------------------------------------------------------------------------
%       An example table
%-------------------------------------------------------------------------------
\begin{table}[p]
\begin{center}
\begin{tabular}{||c|rrrr|rrrr||}
\hline
Label & $\eta^u_{LL}$ & $\eta^u_{LR}$ & $\eta^u_{RL}$ & $\eta^u_{RR}$ & 
        $\eta^d_{LL}$ & $\eta^d_{LR}$ & $\eta^d_{RL}$ & $\eta^d_{RR}$ \\ 
\hline\hline
VV&  $+1$&$+1$&$+1$&$+1$&
     $+1$&$+1$&$+1$&$+1$ \\
AA&  $+1$&$-1$&$-1$&$+1$&
     $+1$&$-1$&$-1$&$+1$ \\
VA&  $+1$&$-1$&$+1$&$-1$&
     $+1$&$-1$&$+1$&$-1$ \\
X1&  $+1$&$-1$&$ 0$&$ 0$&
     $+1$&$-1$&$ 0$&$ 0$ \\
X2&  $+1$&$ 0$&$+1$&$ 0$&
     $+1$&$ 0$&$+1$&$ 0$ \\
X3&  $+1$&$ 0$&$ 0$&$+1$&
     $+1$&$ 0$&$ 0$&$+1$ \\
X4&  $ 0$&$+1$&$+1$&$ 0$&
     $ 0$&$+1$&$+1$&$ 0$ \\
X5&  $ 0$&$+1$&$ 0$&$+1$&
     $ 0$&$+1$&$ 0$&$+1$ \\
X6&  $ 0$&$ 0$&$+1$&$-1$&
     $ 0$&$ 0$&$+1$&$-1$ \\
U1&  $+1$&$-1$&$ 0$&$ 0$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U2&  $+1$&$ 0$&$+1$&$ 0$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U3&  $+1$&$ 0$&$ 0$&$+1$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U4&  $ 0$&$+1$&$+1$&$ 0$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U5&  $ 0$&$+1$&$ 0$&$+1$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U6&  $ 0$&$ 0$&$+1$&$-1$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
\hline
\end{tabular}
\caption{The 30 scenarios for a better life considered in this paper.
         Each row of this table corresponds to two different scenarios for
         overall interference signs $\epsilon=+1$ and $\epsilon=-1$, 
         respectively.}
  \label{tab-models}
\end{center}
\end{table}


==> do <==
#!/bin/csh -f
#
#       To run LaTeX and BibTeX on a given LaTeX source file
#       -> Part of LaTeX4zeus, added in version pre-1.0 <-
#
#       Author: U.Katz, Univ. Bonn, April 2000
#               Bug reports etc. to katz@physik.uni-bonn.de
#
#-------------------------------------------------------------------------------
#   Check arguments
#-------------------------------------------------------------------------------
set prog = 'DESY-06-226'
#
set rdct1 = '/dev/tty'
set rdctb = '/dev/tty'
set rdct2 = '/dev/null'
set rdct3 = '/dev/null'
set rdctd = '/dev/tty'
set ltcom = 'latex'
while ( $#argv > 0 )
  switch ( $argv[1] )
  case -q:
  case -Q:
    set rdct1 = '/dev/null'
    set rdctb = '/dev/null'
    set rdctd = '/dev/null'
    breaksw
  case -m:
  case -M:
    breaksw
  case -v:
  case -V:
    set rdct2 = '/dev/tty'
    set rdct3 = '/dev/tty'
    breaksw
  case -h:
  case -H:
    which hugelatex >& /dev/null
    set check = $status
    if ( $check == 0 ) then
      set ltcom = 'hugelatex'
    else
      echo "WARNING: hugelatex not available. Using latex."
      set ltcom = 'latex'
    endif
    breaksw
  default:
    goto usage
    breaksw
  endsw
  shift
end
#-------------------------------------------------------------------------------
#   First latex run
#-------------------------------------------------------------------------------
echo " ==> Calling LaTeX"
echo "" >> ${prog}.l4l
echo " ==> Calling LaTeX" > ${prog}.l4l
echo " -----------------" >> ${prog}.l4l
$ltcom ${prog}.tex |& tee -a ${prog}.l4l >& $rdct1 ||\
  (echo " First LaTeX run failed (see transcript file ${prog}.log)"; exit)
echo "" >> ${prog}.l4l
echo " ==> LaTeX log file (call 1)" >> ${prog}.l4l
echo " ---------------------------" >> ${prog}.l4l
cat ${prog}.log >> ${prog}.l4l
#-------------------------------------------------------------------------------
#   bibtex run
#-------------------------------------------------------------------------------
echo " ==> Calling BibTeX"
echo "" >> ${prog}.l4l
echo " ==> Calling BibTeX" >> ${prog}.l4l
echo " ------------------" >> ${prog}.l4l
bibtex ${prog} |& tee -a ${prog}.l4l >& $rdctb ||\
  (echo " BiBTeX run failed (see transcript file ${prog}.blg)"; exit)
echo "" >> ${prog}.l4l
echo " ==> BiBTeX log file" >> ${prog}.l4l
echo " -------------------" >> ${prog}.l4l
cat ${prog}.blg >> ${prog}.l4l
#-------------------------------------------------------------------------------
#   Second latex run
#-------------------------------------------------------------------------------
echo " ==> Calling LaTeX"
echo "" >> ${prog}.l4l
echo " ==> Calling LaTeX" >> ${prog}.l4l
echo " -----------------" >> ${prog}.l4l
$ltcom ${prog}.tex |& tee -a ${prog}.l4l >& $rdct2 ||\
  (echo " Second LaTeX run failed (see transcript file ${prog}.log)"; exit)
echo "" >> ${prog}.l4l
echo " ==> LaTeX log file (call 2)" >> ${prog}.l4l
echo " ---------------------------" >> ${prog}.l4l
cat ${prog}.log >> ${prog}.l4l
#-------------------------------------------------------------------------------
#   Third latex run
#-------------------------------------------------------------------------------
echo " ==> Calling LaTeX"
echo "" >> ${prog}.l4l
echo " ==> Calling LaTeX" >> ${prog}.l4l
echo " -----------------" >> ${prog}.l4l
$ltcom ${prog}.tex |& tee -a ${prog}.l4l >& $rdct3 ||\
  (echo " Third LaTeX run failed (see transcript file ${prog}.log)"; exit)
echo "" >> ${prog}.l4l
echo " ==> LaTeX log file (call 3)" >> ${prog}.l4l
echo " ---------------------------" >> ${prog}.l4l
cat ${prog}.log >> ${prog}.l4l
#-------------------------------------------------------------------------------
#   Finally call dvips
#-------------------------------------------------------------------------------
echo " ==> Calling dvips"
echo "" >> ${prog}.l4l
echo " ==> Calling dvips" >> ${prog}.l4l
echo " -----------------" >> ${prog}.l4l
dvips -t a4 ${prog}.dvi -o |& tee -a ${prog}.l4l >& $rdctd
set sta = $status
if ( $sta != 0 ) then
  echo " dvips failed - status" $sta
  echo " dvips failed - status" $sta >> ${prog}.log
  exit
endif

gv -portrait DESY-06-226.ps &
#-------------------------------------------------------------------------------
#   Usage information
#-------------------------------------------------------------------------------
usage:
cat <<EOF
 Usage:   t_lp [options]
          ----------------------
          Options:
          -q   quiet: i.e. no output to terminal
          -m   medium: output of first latex command, bibtex
               and dvips to terminal (default)
          -v   verbose: all output to terminal
          -h   to use hugelatex instead of latex (if available)

 Note that all command output is collected in file lp.l4l,
 independent of the choice of options.

EOF

exit

